Layer Swapping for Zero-Shot Cross-Lingual Transfer in Large Language Models

Model merging, such as model souping, is the practice of combining different models with the same architecture together without further training. In this work, we present a model merging methodology that addresses the difficulty of fine-tuning Large Language Models (LLMs) for target tasks in non-English languages, where task-specific data is often unavailable. We focus on mathematical reasoning and without in-language math data, facilitate cross-lingual transfer by composing language and math capabilities. Starting from the same pretrained model, we fine-tune separate "experts" on math instruction data in English and on generic instruction data in the target language. We then replace the top and bottom transformer layers of the math expert directly with layers from the language expert, which consequently enhances math performance in the target language. The resulting merged models outperform the individual experts and other merging methods on the math benchmark, MGSM, by 10% across four major languages where math instruction data is scarce. In addition, this layer swapping is simple, inexpensive, and intuitive, as it is based on an interpretative analysis of the most important parameter changes during the fine-tuning of each expert. The ability to successfully re-compose LLMs for cross-lingual transfer in this manner opens up future possibilities to combine model expertise, create modular solutions, and transfer reasoning capabilities across languages all post hoc.

==> section/results_old.tex <==
\section{Empirical Results} \label{results}

%\ben{I would move here the experimental detail on: what languages you're experimenting with, what dataset you're using, how much you're training each experts}

Given the potential use cases of such a method, there are numerous ways in which we can measure the success of such a method. %\ben{rephrase sentence}. 
We conduct numerous experiments with the fine-tuned experts discussed in Section~\ref{experts}, where we select the three best math experts, and the three best experts for each of Swahili, Japanese, Telugu, Bengali. For each language, that gives us nine pairs to evaluate. 
% \ben{you need to justify why we want/need to have 3 expert for each case}

\subsection{Baselines} \label{baselines}

We present numerous baselines to contextualize the performance of our method.%\ls. 
%\ben{\textit{to give more intuition about why you pick these baselines, Suggestion:} If our layer swapping technique is effective, we expect our resulting model to outperform the initial model we use, as well as each individual expert on their own.}
%\ben{Therefore,} 
We first present the MGSM scores of the pre-trained \llama base model as well as the individual experts that were merged, in order to display the effect of merging disparate experts.  In addition, we present an alternative for Swahili where instead of post hoc model merging, we mix the language and math datasets and do a single fine-tuning run with samples from both. Instead of training two experts, each on 30-40k samples, the joint SFT is over the union (80k samples).

\input{tables/swh_baselines}

For model merging methods, we compare \ls to the classic model souping \citep{Wortsman2022}, where all parameters are simple averages of the two experts. For each, we also evaluate adjusting for the magnitude of change from the base model to the expert by doing a weighted average. Using notation from Section~\ref{vis}, the resulting weight of each expert is the inverse of the average MAV for all rows in all $\displaystyle \tW_\Delta$ for that expert. This weighted averaging sometimes yields better performance than the uniform soup, but never by very much. The second merging baseline we evaluate for Swahili is TIES-merging \citep{Yadav2023}, which resolves interference between experts by sequentially trimming conflicting values, determining the sign of each weight, and then merging the resulting weights.

\subsection{Results}

In Table~\ref{swh-stats}, we show the results MGSM benchmark across a number of different runs for each setting with Swahili as the target language. Here, we find \ls to consistenly outperform baselines. For each of the nine pairs, the default \ls configuration scores higher on the Swahili split of the MGSM benchmark than either of the individual experts, the souped experts, or the TIES-merged experts. This tremendous consistency also followed for many other configurations. For the Swahili and math joint SFT, we are also able to achieve comparably high results, with numerous checkpoints reaching the average range of our \emph{layer-swapped} models. However, the maximum performance of these checkpoints lagged the best \emph{layer-swapped} pairs by over 4 percentage points. This means that the ceiling for cross-lingual transfer is significantly higher with this methodology than simply mixing datasets together.

\input{tables/fourlangs_tbl}

For languages other than Swahili, we see in Table~\ref{stats} that model souping is ineffective for merging models, as performance is often below the MGSM scores of the math experts and the ceiling and average of is consistently lower than \ls. This method was certainly most effective for Swahili and Telugu, where \llama was less good to begin with. We also note that these are the languages where the math experts, on their own, were less good as well. While we only evaluate four languages in this work, we conjecture that this method is most effective for lower-resource languages. Part of that is potentially the difficulty to boost language capabilities with low-data SFT when \llama was already pre-trained on more tokens in that language. Additionally, for higher-resource languages, natural cross-lingual transfer occurs more directly when fine-tuning on English math data. For Japanese, in particular, we see that the math experts were better than our \emph{layer-swapped} models on average~\footnote{We note that our Japanese experts were the weakest; the increase in performance across \belebele, \flores, MBPP, and MMLU after SFT were minimal. %(See Appendix~\ref{expertresults})
Perhaps there are better data or hyperparameter SFT setups that would enable \ls to more effectively transfer from the math expert.}.

\input{tables/soupswap.tex}



Given multiple experts, this method can also combine with other model merging methods when there are more than one language or math expert. We experiment souping with souping the three experts for each of the languages before \ls with a soup of the three math experts and present results in Table~\ref{soupswap}. In the rightmost column of that table, we also present results from souping a 12-model multilingual soup with the three-model math soup. These larger soups do not consistently work better with \ls than non-souped expert pairs on average (let alone the best pair), but shows that it is feasible and that there is therefore a wide realm of possibilities.
